Situated Mapping of Sequential Instructions to Actions with Single-step Reward Observation

We propose a learning approach for mapping context-dependent sequential instructions to actions. We address the problem of discourse and state dependencies with an attention-based model that considers both the history of the interaction and the state of the world. To train from start and goal states without access to demonstrations, we propose SESTRA, a learning algorithm that takes advantage of single-step reward observations and immediate expected reward maximization. We evaluate on the SCONE domains, and show absolute accuracy improvements of 9.8%-25.3% across the domains over approaches that use high-level logical representations.

==> analysis.tex <==
\section{Analysis}
\label{sec:analysis}

\begin{table}
\begin{footnotesize}
\begin{center}
\begin{tabular}{|p{2cm}|c|c|c|} \hline
Class & \textsc{Alchemy} & \textsc{Scene} & \textsc{Tangrams} \\ \hline
multi-turn ref. & & 5 & 13 \\ \hline
impossible multi-turn ref. & & 5 & 13 \\ \hline
unclear label & & 19 & 12 \\ \hline
in-turn ref. & & 13 & 7 \\ \hline
misunderstands task & & 7 & 3 \\ \hline
\end{tabular}
\end{center}
\end{footnotesize}
\caption{Counts of common errors in the three domains. }
\label{tab:analysis}
\end{table}

\paragraph{Error Analysis}
We analyze the performance of our best models with respect to errors that occur on an instruction-level, i.e. when the agent is provided with the correct initial state.
We observe \as{fifty} examples in each domain.
Table~\ref{tab:analysis} shows the counts of major error categories across the domains.
We consider errors with resolving references both from previous utterances (multi-turn) and in the environment (in-turn).
Some multi-turn reference resolution errors are due to the model not having access to previous world states.
For example, in \textsc{Tangrams}, the instruction \nlstring{put it back in the same place} refers to a previously-removed item.
Because the agent only has access to the world state after following this instruction, it does not observe what kind of item was previously removed, and therefore cannot correctly identify which item it should add back.
Additionally, we find that a significant number of errors are due to ambiguous or incorrect instructions.
For example, the \textsc{Scene} instruction \nlstring{person in green appears on the right end} is ambiguous.
In the data, it is interpreted as \nlstring{person in green} referring to a person already in the environment, who moves to the 10th position.
However, it can also be interpreted as a new person in green appearing in the 10th position.

\begin{figure*}[t]
\fbox{
\centering
\begin{minipage}{0.45\linewidth}
	\includegraphics[width=\linewidth,clip,trim=65 75 65 20,page=1, right]{figs/attention} \\
\end{minipage}
\begin{minipage}{0.45\linewidth}\vspace{9mm}
	\includegraphics[width=0.6\linewidth,clip,trim=70 125 550 125,page=2, left]{figs/attention} \\
\end{minipage}}
\caption{Attention}
\label{fig:attention}	
\end{figure*}


\paragraph{Attention Analysis}
Figure~\ref{fig:attention} shows attention distributions for an example in \textsc{Alchemy}.
The supplementary material contains more examples of attention.
